5G-WAVE: A Core Network Framework with Decentralized Authorization for Network Slices

5G mobile networks leverage Network Function Virtualization (NFV) to offer services in the form of network slices. Each network slice is a logically isolated fragment constructed by service chaining a set of Virtual Network Functions (VNFs). The Network Repository Function (NRF) acts as a central OpenAuthorization (OAuth) 2.0 server to secure inter-VNF communications resulting in a single point of failure. Thus, we propose 5G-WAVE, a decentralized authorization framework for the 5G core by leveraging the WAVE framework and integrating it into the OpenAirInterface (OAI) 5G core. Our design relies on Side-Car Proxies (SCPs) deployed alongside individual VNFs, allowing point-to-point authorization. Each SCP acts as a WAVE engine to create entities and attestations and verify incoming service requests. We measure the authorization latency overhead for VNF registration, 5G Authentication and Key Agreement (AKA), and data session setup and observe that WAVE verification introduces 155ms overhead to HTTP transactions for decentralizing authorization. Additionally, we evaluate the scalability of 5G-WAVE by instantiating more network slices to observe 1.4x increase in latency with 10x growth in network size. We also discuss how 5G-WAVE can significantly reduce the 5G attack surface without using OAuth 2.0 while addressing several key issues of 5G standardization.

==> motivation.tex <==
\section{Motivation}

In this section, we describe our two-stage motivation for building the 5G-WAVE integrated platform. Firstly, we discuss how specific OAuth attack vectors are addressed in Table~\ref{tbl:oauthvswwave}. Secondly, to illustrate how the proposed design improves the flexibility and security of the 5G core, we reference Key Issues (KIs) from the 3GPP standardization in Table~\ref{tbl:keyissues}. 

\subsection{Comparing 5G-OAuth and 5G-WAVE}

%As commercial 5G networks continue to expand, security features of the deployments require more stringent scrutiny. An overview of the required security capabilities and functionalities for a fully functional 5G deployment is provided in \cite{3gpp33501}. Both industry and academic researchers have investigated the mutual authentication and authorization between the UE and the 5G core~\cite{koutsos20195g,basin2018formal}. However, there has been limited research into potential improvements for 5G core SBA security that explores inter-VNF authorization.


\begin{comment}
\begin{table}[b]
\centering
% \small\selectfont
\caption{Comparing the detection and mitigation capabilities of the standardized 5G-OAuth framework with the 5G-WAVE integrated platform}
\label{tbl:oauthvswwave}
\begin{tabular}
{|c|P{0.08\linewidth}|P{0.1\linewidth}|P{0.08\linewidth}|P{0.11\linewidth}|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Attack Type}}} & \multicolumn{2}{c|}{\footnotesize \textbf{5G + OAuth}}                                       & \multicolumn{2}{c|}{ \footnotesize \textbf{5G + WAVE}}                       \\ 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c}{\scriptsize \textbf{Detect}} & \multicolumn{1}{c|}{\scriptsize \textbf{Mitigate}} & \multicolumn{1}{c}{\scriptsize \textbf{Detect}} & \multicolumn{1}{c|}{\scriptsize \textbf{Mitigate}} \\ \hline    

\small Access Permission & \cellcolor{red!10} x & \cellcolor{red!10} x  & $\cellcolor{green!10}\checkmark$  & $\cellcolor{green!10}\checkmark$  \\ \hline

\small Data Manipulation  & \cellcolor{red!10} x & \cellcolor{red!10} x & \cellcolor{green!10}$\checkmark$ & \cellcolor{green!10} $\checkmark$ \\ \hline    

\small Auth-Flooding & \cellcolor{green!10} $\checkmark$ & \cellcolor{red!10}x & \cellcolor{green!10}$\checkmark$  & \cellcolor{green!10}$\checkmark$ \\ \hline

\small Denial of Service  & \cellcolor{green!10} $\checkmark$ & \cellcolor{red!10}x & \cellcolor{green!10} $\checkmark$  & \cellcolor{green!10} $\checkmark$  \\ \hline

\small De-Authentication                             & \cellcolor{red!10}x & \cellcolor{red!10}x  & \cellcolor{green!10} $\checkmark$ & \cellcolor{green!10} $\checkmark$  \\ \hline

\small Service Scanning                            & \cellcolor{green!10} $\checkmark$   & \cellcolor{red!10}x  & \cellcolor{green!10} $\checkmark$ & \cellcolor{green!10} $\checkmark$  \\ \hline

\small Data Sniffing                        & \cellcolor{red!10}x & \cellcolor{red!10}x  & \cellcolor{red!10}x & \cellcolor{green!10} $\checkmark$  \\ \hline

\small Token Replay                               & \cellcolor{red!10}x & \cellcolor{red!10}x  & \cellcolor{green!10} $\checkmark$ & \cellcolor{green!10} $\checkmark$ \\ \hline
\end{tabular}
\end{table}    
\end{comment}

\begin{table}[b]
\centering
% \small\selectfont
\caption{Comparing the detection and mitigation capabilities of the standardized 5G-OAuth framework with the 5G-WAVE integrated platform ($\checkmark$: addressed, \FilledTriangleUp: addressed with additional client-side configuration, x: vulnerable)}
\label{tbl:oauthvswwave}
\begin{tabular}
{l|c|c}
%\hline
\textbf{Attack Type} & \textbf{5G-OAuth} & \textbf{5G-WAVE} \\ \hline \hline
%\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c}{\scriptsize \textbf{Detect}} & \multicolumn{1}{c|}{\scriptsize \textbf{Mitigate}} & \multicolumn{1}{c}{\scriptsize \textbf{Detect}} & \multicolumn{1}{c|}{\scriptsize \textbf{Mitigate}} \\ \hline    

\small Authorization Code Injection & \cellcolor{orange!40} \FilledTriangleUp & $\cellcolor{green!10}\checkmark$  \\ %\hline

\small Access Token Leakage & \cellcolor{orange!40} \FilledTriangleUp & \cellcolor{green!10} $\checkmark$ \\ %\hline    

\small Credential Phishing Attacks & \cellcolor{orange!40} \FilledTriangleUp  & \cellcolor{green!10}$\checkmark$ \\ %\hline

\small Authorization Flooding  & \cellcolor{red!30} x & \cellcolor{green!10} $\checkmark$  \\ %\hline

\small Access Token Hijacking & \cellcolor{orange!40} \FilledTriangleUp  & \cellcolor{green!10} $\checkmark$  \\ \hline

%\small Service Scanning & \cellcolor{green!10} $\checkmark$ & \cellcolor{green!10} $\checkmark$  \\ \hline

\end{tabular}
\end{table}

To ensure inter-slice and intra-slice security, it is essential to move the 5G core SBA towards a Zero-Trust Architecture (ZTA) \cite{Rose2020Aug}. One of the key principles of ZTA is `Never Trust, Always Verify' \cite{Rose2020Aug}, which demands all network entities to be authenticated, authorized, and continuously verified before being granted access to resources. Towards achieving SBA-domain security in 5G, 3GPP has standardized OAuth 2.0 as an authorization framework for VNF service access. Within this framework, the NRF acts an authorization server that distributes access tokens to service consumer VNFs~\cite{3gpp33501,3gpp29510}. Either directly or as a result of misconfiguration, OAuth 2.0 is vulnerable to the attack types listed in Table~\ref{tbl:oauthvswwave}.

When OAuth 2.0 is replaced with a decentralized approach, we remove the dependency on the NRF as a central authorization server. Ultimately, each VNF service provider will become both the authorization and resource server for their own services. To realize this idea, our decentralized authorization framework of choice is WAVE. It has been shown that WAVE performs better than traditional authorization frameworks by providing stronger security guarantees with comparable performance~\cite{Andersen2019}. %It fulfills the 5G core security requirements \cite{3gpp33501} while increasing the flexibility of deployment. 

In WAVE, access is granted in the form of encrypted attestations rather than tokens. As a result, the resource requester and resource provider are bound to each other in the WAVE authorization chain without involving a third-party server. These attestations can be stored in a distributed manner using horizontally scalable servers without compromising system security. The critical security features provided by incorporating WAVE into the 5G core are listed below.

\begin{itemize}
    \item Confidentiality, integrity, and replay protection are supported for inter-VNF communication.
    \item The 5G core network slice topology in each administrative domain is maintained separately. Thus, for Multi-Operator Networks (MNOs), the VNF topologies are hidden from entities in different trust domains.
    \item Service consumers/providers are mutually authenticated. 
    \item Instead of relying on an authorization server, the service request messages will be validated by the service provider VNFs. Invalid or unauthorized messages will be rejected or discarded according to the protocol specification.
\end{itemize}

A comparison of the 5G-OAuth and 5G-WAVE is provided in Table~\ref{tbl:oauthvswwave}. The specific attack vectors are explained below.

As a Man-in-the-Middle (MiTM) attacker, adversaries can perform \textbf{authorization code injections}, \textbf{access token hijacking} and take advantage of \textbf{token leakages} in the OAuth 2.0 framework~\cite{RFC6819O63online,draftiet79online,yang2016model}. Without additional client-side security implemented on the VNFs (e.g., URL redirects, TLS), the 5G core remains vulnerable to these OAuth 2.0 attack vectors. On the other hand, WAVE prevents these attacks by removing the reliance on access tokens. By extension, this no longer requires the employment of risk-inducing information elements such as authorization codes and access scopes.

As a centralized authorization server, the NRF is vulnerable against \textbf{authorization flooding} attacks. Adversaries can execute a Distributed Denial of Service (DDoS) by generating a high volume of access token requests directed at the NRF. With the decentralization provided by the 5G-WAVE integration, this vulnerability (i.e., NRF as OAuth 2.0 server) is removed. 

Adversaries using \textbf{phishing attacks} will impersonate a legitimate service requester to obtain illegal access tokens and/or access credentials from legitimate OAuth 2.0 entities. However, WAVE uses custom entities adjacent to each 5G core VNF to ensure their authenticity. As a result, any impersonator not accompanied by a WAVE entity will not be able to infiltrate the authorization chain of the 5G-WAVE integrated platform.

Several attacks from Table~\ref{tbl:oauthvswwave} can be addressed by additional client-side configuration. However this requires additional policies, development effort and expertise. With the 5G-WAVE integrated platform, all the attack types are addressed out-of-the-box. This enables mobiles operators to focus on deployment without concern for the underlying security.

\begin{comment}
\begin{itemize}
    \item \textbf{Access token injection with token ID replay.} If an attacker is able to intercept the access tokens issued to a client, then they can impersonate that client and gather privileged data with replay attacks. To do so, the attacker will attach the intercepted token to rogue HTTP transactions and issue them to the service provider to obtain information within the token's scope of access. %There is no way to detect such an injection attack on the OAuth protocol level since the token is issued without any binding to the transaction or the particular user agent.
    \item \textbf{Man-in-the-Middle (MitM) Attack.} A MiTM attacker who can eavesdrop and manipulate tokens, can compromise the integrity of inter-VNF communications in the core network.
    \item \textbf{Central point of attack.} The dependency on a central authorization server leaves the system vulnerable to attacks. With a single point of failure, adversaries can focus their attack vectors toward the NRF to either compromise or hinder its functionalities. This can result in malicious or misconfigured authorization tokens being distributed to the VNFs.
\end{itemize}
\end{comment}



\subsection{3GPP Key Issues}

\begin{table}[b]
\centering
% \small\selectfont
\caption{Summary of 3GPP key issues addressed by the 5G-WAVE integrated platform ($\checkmark$: directly addressed, \FilledTriangleUp: addressed with proper configuration, $\hourglass$: future work)}
\label{tbl:keyissues}
% \begin{tabular}{p{0.1\columnwidth}|p{0.3\columnwidth}|p{0.2\columnwidth}}
\begin{tabular}{c|c|c|c}
 \textbf{3GPP \#} & \textbf{KI \#} & \textbf{Description} & \textbf{5G-WAVE} \\
 \hline \hline
 33.813~\cite{3gpp33813} & 5 & token handling between slices & \cellcolor{green!10} $\checkmark$ \\
 33.886~\cite{3gpp33886} & 2 & temporary slice authorization & \cellcolor{orange!40} \FilledTriangleUp \\
 33.874~\cite{3gpp33874} & 3 & AF authorization & \cellcolor{orange!40} \FilledTriangleUp \\
 33.813~\cite{3gpp33813} & 1 & slice-specific authorization & \cellcolor{red!30} $\hourglass$ \\
 \hline
\end{tabular}
\end{table}

\textbf{[33.813 KI 5]} The NRF can be deployed at different administrative hierarchies (e.g., Public Land Mobile Network level, shared-slice level, slice-specific level). The tokens distributed by the NRF can be used to access services of the same type of VNF service providers across multiple slices. This can lead to illegal access requests since different network slices may have alternative service consumption policies for their VNF types. The 5G-WAVE integrated platform directly addresses this KI as it removes the need for tokens altogether.

\textbf{[33.886 KI 2]} For the graceful termination of data sessions, UEs are allowed access to temporary slices. This requires efficient authentication and authorization mechanisms to moderate access to such slices. By creating a joint authorization chain between the UE's current network slice and target temporary slice, authorized access can be provided with the 5G-WAVE integrated platform. 

\textbf{[33.874 KI 3]} External Application Functions (AFs)~\cite{3gpp29517} can be exposed to the 5G core SBA for carrying out custom operator functions. Without proper authentication and authorization, malicious AFs can gain access to sensitive information by accessing network slices. The operator can attach the AFs to the 5G-WAVE integrated authorization chain to seamlessly incorporate them in the transitive delegation hierarchy. Thus, the service provider VNFs can directly provide authorization to AFs for service consumption.

\textbf{[33.813 KI 1]} Network slice-specific authentication and authorization has become a fundamental requirement. To address this KI, 3GPP has already standardized the Network Slice-Specific Authentication and Authorization Function (NSSAAF)~\cite{3gpp29526}. This additional VNF will serve as an independent authentication and authorization server for moderating access to individual slices. Currently, the 5G-WAVE integrated platform cannot directly be used to address this KI. As a future work, we plan to store slice-specific metadata inside the wSCPs that are hosting the WAVE entities. Ultimately, it will be possible to keep track of the VNF authorizations along with their network slices. 











